CompilerGym: Robust, Performant Compiler Optimization Environments for AI Research

Interest in applying Artificial Intelligence (AI) techniques to compiler optimizations is increasing rapidly, but compiler research has a high entry barrier. Unlike in other domains, compiler and AI researchers do not have access to the datasets and frameworks that enable fast iteration and development of ideas, and getting started requires a significant engineering investment. What is needed is an easy, reusable experimental infrastructure for real world compiler optimization tasks that can serve as a common benchmark for comparing techniques, and as a platform to accelerate progress in the field. We introduce CompilerGym, a set of environments for real world compiler optimization tasks, and a toolkit for exposing new optimization tasks to compiler researchers. CompilerGym enables anyone to experiment on production compiler optimization problems through an easy-to-use package, regardless of their experience with compilers. We build upon the popular OpenAI Gym interface enabling researchers to interact with compilers using Python and a familiar API. We describe the CompilerGym architecture and implementation, characterize the optimization spaces and computational efficiencies of three included compiler environments, and provide extensive empirical evaluations. Compared to prior works, CompilerGym offers larger datasets and optimization spaces, is 27x more computationally efficient, is fault-tolerant, and capable of detecting reproducibility bugs in the underlying compilers. In making it easy for anyone to experiment with compilers - irrespective of their background - we aim to accelerate progress in the AI and compiler research domains.

==> appendices/artifact-evaluation.tex <==
\section{Artifact Appendix}

\lstset{%
    frame=l,
    rulecolor=\color{red},
}

\subsection{Abstract}

Our artifact comprises source code and pre-compiled binaries for CompilerGym,
and instructions to reproduce the nine experiments in the paper.


\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Run-time environment: } Ubuntu 18.04, Fedora 28, Debian 10 or
  newer, or macOS. Python 3.8.
  \item {\bf Experiments: } Computational efficiency benchmarks; autotuning for
  LLVM phase ordering, GCC command line flags, and CUDA loop nests; supervised
  graph learning; and reinforcement learning for LLVM phase ordering.
  \item {\bf How much disk space required (approximately)?: } 20GB.
  \item {\bf How much time is needed to prepare workflow (approximately)?: } 15
  minutes.
  \item {\bf How much time is needed to complete experiments (approximately)?: }
  3 hours.
  \item {\bf Publicly available?: } Yes. \url{https://compilergym.ai}
\end{itemize}
}


\subsection{Description}

\subsubsection{How delivered}

The artifact is available from:\\*
\url{https://doi.org/10.5281/zenodo.5784251}.

\subsubsection{Hardware dependencies}

We recommend a minimum of 64GB RAM. We used a commodity desktop machine equipped
with a AMD Ryzen 9 3900X CPU and NVIDIA 2080 GPU to generate the compute time
estimates in this document.
%
A CUDA-equipped GPU is required for one of the experiments
(Section~\ref{subsection:autotuning-loop-tool}).
%
The following experiments contain runtime measurements and so will produce
different vakyes on your system:
Sections~\ref{subsection:computational-efficiency},
\ref{subsection:observation-spaces-efficiency},
\ref{subsection:autotuning-llvm}, and~\ref{subsection:autotuning-loop-tool}. The
remainder of the experiments are hardware-agnostic.


\subsubsection{Software dependencies}

All experiments require Python 3.8. We recommend using anaconda to prevent
interference with your system Python.
%
Docker is required for one of the experiments
(Section~\ref{subsection:autotuning-gcc}).


\subsection{Installation}

(Optional) Use conda\footnote{If not already available, see the documentation
for installation
instructions:\\*\url{https://docs.conda.io/projects/conda/en/latest/user-guide/install/index.html}}
to create a clean Python environment:
%
\begin{lstlisting}
conda create -y -n compiler_gym python=3.8
conda activate compiler_gym
\end{lstlisting}
%
\noindent
Confirm that your environment is using Python 3.8:
%
\begin{lstlisting}
python --version
\end{lstlisting}
%
\noindent
Next, install the \cg{} library using:
%
\begin{lstlisting}
python -m pip install -U compiler_gym
\end{lstlisting}
%
\noindent
Either download the artifact archive linked above, or clone the repository to
get the most recent version using:
%
\begin{lstlisting}
git clone \
    https://github.com/facebookresearch/CompilerGym.git
\end{lstlisting}
%
\noindent
Change to the examples directory and install the dependencies using:
\begin{lstlisting}
cd CompilerGym/examples
python setup.py install
\end{lstlisting}
%
\noindent
The remainder of this document requires that the user remains in the
\texttt{\scriptsize CompilerGym/examples} directory.


\subsection{Experiments}

This section describes how to reproduce all of the experiments in the paper. The
workflow, evaluation, and customization steps of each experiment is described in
turn.

\vspace{1em}
\noindent
\textbf{(Optional) Getting Started with CompilerGym}

Before running the experiments below we recommend navigating to
\url{https://compilergym.ai/getting_started} and clicking the ``Open in Colab''
button to launch an interactive webpage that describes the main CompilerGym
concepts and APIs. It takes approximately 20 minutes to complete.

\vspace{1em}
\noindent
\textbf{Sections~\ref{subsection:computational-efficiency}
and~\ref{subsection:observation-spaces-efficiency}: Computational Efficiency}

\emph{Workflow:} The following script benchmarks the computation times of the
three environment operations (startup, initialization, and step), and each of
the eight observation spaces:
%
\begin{lstlisting}
python -m op_benchmarks run --n=200
\end{lstlisting}
%
\noindent
where \texttt{\footnotesize --n} is the number of runtimes to collect for each
type of operation. Collecting \texttt{\footnotesize --n=200} measurements will
take about 10 minutes. In the paper we use \texttt{\footnotesize --n=1000000}.

\emph{Evaluation:} Aggregate measurements and compare the runtimes to
Table~\ref{table:llvm-op-costs} and Table~\ref{table:llvm-observation-spaces}
using:
%
\begin{lstlisting}
python -m op_benchmarks info
\end{lstlisting}

\vspace{1em}
\noindent
\textbf{Section~\ref{subsection:autotuning-llvm}: Autotuning LLVM Phase
Ordering}

\emph{Workflow:} Run a single autotuning experiment using:
%
\begin{lstlisting}
export AUTOTUNER=nevergrad; TARGET=codesize; \
python -m llvm_autotuning.tune -m \
    experiment="${AUTOTUNER}-${TARGET}" \
    autotuner="${AUTOTUNER}" \
    autotuner.optimization_target="${TARGET}" \
    num_replicas=1 \
    autotuner.search_time_seconds=300
\end{lstlisting}
%
where \texttt{\scriptsize AUTOTUNER} is set to one of \texttt{\scriptsize
nevergrad}, \texttt{\scriptsize random}, \texttt{\scriptsize greedy}, or
\texttt{\scriptsize opentuner}; and \texttt{\scriptsize TARGET} is set to one of
\texttt{\scriptsize codesize}, \texttt{\scriptsize binsize}, or
\texttt{\scriptsize runtime}. Run all 12 combinations of autotuner and target to
reproduce the full suite of experiments in
Section~\ref{subsection:autotuning-llvm}.

The above command will take about 6 minutes to complete. Compared to the
experiment in the paper each autotuner is run only once and with a search budget
of 5 minutes instead of one hour. To replicate the full experiment from
Section~\ref{subsection:autotuning-llvm}, taking about 12 hours, run:
%
\begin{lstlisting}
export AUTOTUNER=nevergrad; TARGET=codesize; \
python -m llvm_autotuning.tune -m \
    experiment="${AUTOTUNER}-${TARGET}" \
    autotuner="${AUTOTUNER}" \
    autotuner.optimization_target="${TARGET}" \
    num_replicas=10 \
    autotuner.search_time_seconds=3600
\end{lstlisting}

\emph{Evaluation:} Aggregate and compare to Table~\ref{table:llvm-autotuning}
using:
%
\begin{lstlisting}
python -m llvm_autotuning.info
\end{lstlisting}

\emph{Customization:} The experiment is configurable through several command
line arguments described in \texttt{\scriptsize llvm\_autotuning/README.md}.
Example customizations include \texttt{\scriptsize
autotuner.search\_time\_seconds} to change the search budget, and
\texttt{\scriptsize autotuner.algorithm\_config.episode\_length} to set the
number of steps in Nevergrad environment episodes.


\vspace{1em}
\noindent
\textbf{Section~\ref{subsection:autotuning-gcc}: Autotuning GCC Command Line
Flags}

\emph{Workflow:} Run a small-scale autotuning experiment using:
%
\begin{lstlisting}
python -m gcc_autotuning.tune \
    --gcc_search_budget=100 \
    --pop_size=20 \
    --gcc_search_repetitions=1 \
    --gcc_benchmark=benchmark://chstone-v0/aes,benchmark://chstone-v0/blowfish,benchmark://chstone-v0/dfmul,benchmark://chstone-v0/dfsin,benchmark://chstone-v0/sha
\end{lstlisting}
%
\noindent
Note the final \texttt{\footnotesize --gcc\_benchmark} argument above should
entered as a single line without spaces. This requires docker. If docker is not
installed, use \texttt{\footnotesize --gcc\_bin=/path/to/gcc} to specify the
path to a GCC installation. The above command takes about 12 minutes to complete
and uses fewer benchmarks and a smaller search budget than in the paper. To
replicate the full suite setup from Section~\ref{subsection:autotuning-gcc},
taking about 6 hours, run:
%
\begin{lstlisting}
python -m gcc_autotuning.tune
\end{lstlisting}

\emph{Evaluation:} Aggregate and compare to Table~\ref{table:gcc-autotuning}
using:
%
\begin{lstlisting}
python -m gcc_autotuning.info
\end{lstlisting}

\emph{Customization:} The experiment is configurable through a number of command
line arguments described in \texttt{\scriptsize gcc\_autotuning/README.md}.
Example customizations include \texttt{\scriptsize --gcc\_search\_budget} to
change the search budget, \texttt{\scriptsize --gcc\_bin} to use a different GCC
binary, and \texttt{\scriptsize --gcc\_benchmark} to change the list of programs
used.

\vspace{1em}
\noindent
\textbf{Section~\ref{subsection:autotuning-loop-tool}: Autotuning CUDA Loop
Nests}

\emph{Workflow:} Run a sweep on a CUDA-capable GPU using:
%
\begin{lstlisting}
python -m loop_tool_sweep --device=cuda --k=128
\end{lstlisting}
%
\noindent
This will take approximately 3 minutes to complete. In
Section~\ref{subsection:autotuning-loop-tool} this experiment is repeated using
the following values for \texttt{\scriptsize --k}: 512, 1024, 2048, 4096, and
8192.

\emph{Evaluation:} Compare values logged to stdout to
Figure~\ref{figure:loop-tool-sweep}.

\emph{Customization:} Use \texttt{\scriptsize --k} and \texttt{\scriptsize
--vectorize} to specify the dataset and vectorization sizes, respectively, and
\texttt{\scriptsize --device=cpu} to run on CPU.

\vspace{1em}
\noindent
\textbf{Section~\ref{subsection:sl-offline-dataset}: Learning a Cost Model}

\emph{Workflow:} Train a graph neural network cost model using:
%
\begin{lstlisting}
python -m gnn_cost_model.train \
    --device=cpu --batch_size=4 \
    --num_epoch=10 --dataset_size=100
\end{lstlisting}
%
\noindent
The above command takes around 10 minutes to complete and uses 100 graphs from a
small 3 GB state transition dataset. To replicate the full scale experiment of
Section~\ref{subsection:sl-offline-dataset}, run:
%
\begin{lstlisting}
python -m gnn_cost_model.train --num_epoch=35 \
    --db=https://dl.fbaipublicfiles.com/compiler_gym/state_transition_dataset/2021-11-15-cbench.tar.bz2
    --db_sha256=36dddceca405126a1249c640cba5b678d4a1db3d9298ad7e5f1d
        a2fa4eccfd20
\end{lstlisting}
\noindent
This requires a minimum of 60 GB of RAM and disk space.

\emph{Evaluation:} Compare loss logged to stdout to
Figure~\ref{figure:supervised-learning}.

\emph{Customization:} The training script can be configured through several
command line arguments. List them using:
%
\begin{lstlisting}
python -m gnn_cost_model.train --help
\end{lstlisting}


\vspace{1em}
\noindent
\textbf{Sections~\ref{subsection:rl-algos}, \ref{subsection:rl-training-set},
and~\ref{subsection:rl-observation-spaces}: Reinforcement Learning}

\emph{Workflow:} Train a PPO~\cite{ppo} agent for 1000 episodes using:

\begin{lstlisting}
python -m llvm_rl.train -m \
    experiment=algo \
    agent=ppo \
    num_replicas=1 \
    training.episodes=1000
\end{lstlisting}
%
\noindent
This will take approximately 20 minutes to complete. In the paper, agents are
trained for \texttt{\footnotesize training.episodes=100000} and repeated 10
times (\texttt{\footnotesize num\_replicas=10}).

To train using four different algorithms and evaluating on all test sets
(Section~\ref{subsection:rl-algos}), run:
%
\begin{lstlisting}
python -m llvm_rl.train -m \
    experiment=algo \
    agent=a2c,apex,impala,ppo testing=all
\end{lstlisting}
%
\noindent
To cross-validate the effect of different training and test sets
(Section~\ref{subsection:rl-training-set}), run:
%
\begin{lstlisting}
python -m llvm_rl.train -m \
    experiment=training-set \
    training=csmith,github,tensorflow \
    testing=csmith-github-tensorflow
\end{lstlisting}
%
\noindent
To evaluate the effect of different observation spaces on agents
(Section~\ref{subsection:rl-observation-spaces}), run:
%
\begin{lstlisting}
python -m llvm_rl.train -m \
    experiment=observation-spaces \
    training.episodes=100000 \
    environment="autophase,autophase-with-history, \
        instcount,instcount-with-history"
\end{lstlisting}

\emph{Evaluation:} Run the following command to provide an overview of the
training progress of each of the agents:
%
\begin{lstlisting}
python -m llvm_rl.info train
\end{lstlisting}
%
\noindent
This will print the training time and geometric mean rewards achieved on the
training and validation sets. To summarize agent performance on the holdout test
set(s), run:
%
\begin{lstlisting}
python -m llvm_rl.info test
\end{lstlisting}

\emph{Customization:} There are a large number of configuration options
available for the experiment, configured through command line arguments. These
are described in \texttt{\scriptsize lvm\_rl/README.md}. Example customizations
include \texttt{\scriptsize agent.type} to specify the reinforcement learning
algorithm to use, \texttt{\scriptsize environment.max\_episode\_steps} to fix
the number of steps in each episode, \texttt{\scriptsize
environment.reward\_space} to specify the objective function to optimize for,
and \texttt{\scriptsize training.episodes} to specify the number of episodes to
train for.


\subsection{Uninstallation}

After completing the evaluation of this artifact, you can delete the conda
environment using:
%
\begin{lstlisting}
conda deactivate
conda remove --all --name compiler_gym
\end{lstlisting}
\noindent
This will remove the Python package and any installed dependencies. The
following directories can be removed to tidy up CompilerGym's runtime files and
experimental results:
%
\begin{lstlisting}
rm -rf ~/logs/compiler_gym
rm -rf ~/.local/share/compiler_gym
rm -rf ~/.cache/compiler_gym
\end{lstlisting}

\noindent
Finally, you can delete the directory where you cloned the artifact repository.


==> appendices/op_costs.tex <==
\section{Computational Cost Measurements Further Details}

1M of each operation divided evenly across 1000 benchmarks from each of the 14
datasets. If the dataset has fewer than 1000 benchmarks then they are repeated
to make 1000. Else they were sampled randomly without replacement. For step
measurements, a single episode was used per benchmark, yielding an episode of
length 72 ($\lceil{}\frac{1e^6}{14\times1000}\rceil{}$).


\begin{figure*}
  \centering %
  \includegraphics[width=.95\linewidth]{images/step-time-cdf-datasets-large.pdf}
  \vspace{-1em}
  \caption{%
    Cumulative density plot of step times for datasets, ordered by median step
    time. The difference between the median step of the fastest dataset
    (llvm-stress) and the slowest dataset (cbench) is $9.9\times$.%
  }%
  \label{figure:step-time-cdf-datasets-large}
\end{figure*}

\begin{figure*}
  \centering %
  \includegraphics[width=.95\linewidth]{images/step-time-cdf-cbench-large.pdf}
  \vspace{-3em}
  \caption{%
    Cumulative density plot of step times for each of the 23 programs in
    cBench~\cite{cbench}, ordered by median step time. Wall times measured from
    1M random trials. The difference between the median step times of the
    fastest program (crc32) and the slowest program (ghostbench) is
    560.3$\times$.%
  }%
  \label{figure:step-time-cdf-cbench-large}
\end{figure*}

==> appendices/search.tex <==
\section{Autotuning Experiments Further Details}

We selected the hyperparameters for each autotuning technique through grid search on a holdout set of 100 Csmith programs.

\subsection{Nevergrad}
% Raw data: https://colab.research.google.com/drive/1fs9v1fXc9WB7_Llb8XA-eyvwxsiqs6S_?usp=sharing

We considered 16 optimizers and four fixed episode lengths: 5, 25, 50, 100

\begin{figure*}
  \centering %
  \includegraphics[width=.99\linewidth]{images/nevergrad-grid-search}
  \caption{%
    Hyperparameter sweep of black box optimizers using Nevergrad~\cite{nevergrad}. Error bars show 95\% confidence interval.%
  }%
  \label{figure:nevergrad-grid-search}%
\end{figure*}

==> figures/interaction-diagram.tex <==
\begin{figure}
  \centering %
  \includegraphics[width=.95\linewidth]{images/interaction-diagram}
  \caption{%
    Interaction diagram showing how the environment operations map to backend communication. This design enables the backend to be run on a remote machine, and also provides process isolation in case of a compiler crash.%
  }%
  \label{figure:interaction-diagram}
\end{figure}

==> figures/step-time-cdf-datasets.tex <==
% Raw data: https://colab.research.google.com/drive/1g7XI-dcFSUrAi-WgH7RZCFYIMgTUUKz5?usp=sharing
\begin{figure}
  \centering %
  \includegraphics[width=.95\linewidth]{images/step-time-cdf-datasets.pdf}
  \vspace{-1.5em}
  \caption{%
    Cumulative density plot of step times for benchmarks, grouped by dataset and
    ordered by median step time. Wall times measured from 1M random trials. The
    difference between the median step of the fastest dataset (llvm-stress) and
    the slowest dataset (cbench) is $9.9\times$.%
  }%
  \label{figure:step-time-cdf-datasets}
\end{figure}

==> figures/step-time-cdf.tex <==
\begin{figure}
  \centering %
  \includegraphics[width=.95\linewidth]{images/step-time-cdf.pdf}
  \vspace{-2em}
  \caption{%
    Cumulative density plot of 1M steps.
  }%
  \label{figure:step-time-cdf}
\end{figure}


==> supplementary_material.tex <==
\title{Deep Data Flow: Appendices}

\maketitle

\appendix
\input{appendix/dataflow_problems}
\input{appendix/dataset}
\input{appendix/experimental_setup}
\input{appendix/downstream_tasks}

\bibliography{refs}
\bibliographystyle{iclr2021_conference}


==> tables/api-stability.tex <==
\begin{table*}
  \footnotesize
  \begin{tabular}{l L{4cm} L{8cm}}
    \toprule
    & Examples & Stability \\
    \midrule
    Core Python API & \texttt{env.step()}, \texttt{env.reset()} & Stable. We
    provide full compatibility with Gym~\cite{gym}. Should this interface
    change, we will update and maintain backwards compatibility for a minimum of
    three releases.\\
    % \midrule
    %
    Python API Extensions & \texttt{env.fork()}, \texttt{env.validate()} &
    Stable with dreprecations. Breaking changes will be used sparingly where
    they lead to clear improvements in usability or performance. Any breaking
    change will be preceded by runtime deprecation warnings.\\
    % \midrule
    %
    Compiler Backend Interface & The \texttt{CompilationSession} class &
    Somewhat stable. Breaking changes are planned, and will be preceded by
    deprecation notices in the source code. Early upstreaming is recommended to
    alleviate maintenance burden.\\
    % \midrule
    %
    Compiler Service Implementations & The LLVM C++ codebase & Not Stable.
    Breaking changes can happen at any time during development. There is no API
    stability guarantees. Early upstreaming is strongly recommended to avoid
    breakages.\\
    \bottomrule
  \end{tabular}
  \caption{Stability of the API components, ordered from most to least user facing. \chris{Drop this table as soon as space becomes an issue.}}
  \label{table:api-stability}
\end{table*}

